A Survey of the Usages of Deep Learning in Natural Language Processing

Over the last several years, the field of natural language processing has been propelled forward by an explosion in the use of deep learning models. This survey provides a brief introduction to the field and a quick overview of deep learning architectures and methods. It then sifts through the plethora of recent studies and summarizes a large assortment of relevant contributions. Analyzed research areas include several core linguistic processing issues in addition to a number of applications of computational linguistics. A discussion of the current state of the art is then provided along with recommendations for future research in the field.

==> Applications/captioning.tex <==
\subsection{Image and Video Captioning}

\label{section:captioning}

Image captioning is unique in that it combines the fields of natural language processing and computer vision, encoding information from images and decoding it into text. While the encoding process is out of the scope of this survey, the decoding process, as well as, to some degree, holistic models are briefly discussed here.

The automatic captioning of images has been attempted for many years, gaining popularity following the work of Duygulu et al. \cite{Duygulu2002}. The introduction of neural networks to the field has led to significant advancements in recent years. The first neural models were template based \cite{Kulkarni2013,Yang2016} and search based \cite{Devlin2015a, Devlin2015b}. In the prior, aspects of images were recognized and the different words describing these aspects were then combined in standardized grammatical templates. In the latter, images were compared with those in a database and were each assigned the caption of the most similar image.

%Most early efforts at image captioning were search based and template based. Search-based models \cite{Devlin2015} compared images with ground truth corpora of already captioned images. The most similar image descriptions found within the corpora were assigned as the captions for the query images. On the other hand, template-based models \cite{Kulkarni2013,Yang2016} focused on extracting words or grammatical units from query images. Once all the units were extracted, the image descriptions were assembled by computing the most likely word sequences based on known syntactic templates, assuring the correctness of the final captions' structures.

The epitome of neural captioning models, Google's Neural Image Caption (NIC) algorithm \cite{Vinyals2015b}, used a deep CNN, trained for image classifications purposes, as the encoder and an LSTM network for decoding. Karpathy et al. \cite{Karpathy2015} developed an algorithm capturing alignments between image regions and corresponding segments of words. Hendricks et al. \cite{Hendricks2016} addressed the ability to include unseen words in captions with the Deep Compositional Captioning (DCC) model, composed of a lexical classifier and a language model working together. Xu et al. \cite{Xu2015} introduced image attention, feeding the decoder with dynamic vector representations of the most visually salient attributes. You et al. \cite{You2016} developed a semantic attentional model  by combining top-down and bottom-up image features in a feedback process injected to the LSTM-based language model. Lu et al. \cite{Lu2017} proposed an adaptive attentional model that included a sentinel gate within the LSTM architecture in the decoder, dictating whether to consider the encoding or to generate the next word using the language model alone. Rennie et al. \cite{Rennie2017} proposed the use of reinforcement learning to train a deep neural model for image captioning.

To the best knowledge of the authors, the highest performer on the vision-to-language problem, at the time of writing, uses regional attention and scene-specific contexts \cite{Fu2017}. The algorithm segments a query image into spatial regions at a multi-scale level. Given a binary classifier, the semantic concepts captured in the image regions are considered salient for the algorithm when they are semantically meaningful (they relate to high level concepts), primitive, and contextually rich (they have dependency on other nearby regions). Simultaneously, a scene context vector is computed for the whole image.  The addition of the scene vector  (what the image topic is about) provides extra support to the LSTM architecture as it helps in choosing likely words given a certain image context, or in rejecting unlikely words given the same context.

An extension of image captioning is video captioning \cite{Wu2016}. The recently emerging task is treated nearly identically, analyzing a number of frames rather than a single image \cite{Ballas2015}. The frames are combined between the standard encoder and decoder using (a) recurrent layer(s) \cite{Venugopalan2014, Donahue2015}. Recent approaches use hierarchical recurrent networks to perform this task \cite{Pan2016, Yu2016, Baraldi2017}. These networks implement recurrent layers over several frames, and then implement another such layer over the final outputs of the previous layer, reducing the number of connections to a fraction inversely proportional to the number of frames captured by each recurrent implementation in the previous layer. This significantly decreases the number of units through which gradients must be backpropagated. One novel approach \cite{Guo2016} utilized attention along with 3D convolutions. Future work will surely integrate acoustic processing for better captioning and more extensive tasks such as summarizing movies.

==> CoreIssues/LanguageModeling/early_language_modeling.tex <==
\subsubsection{Early Language Modeling}

\label{section:early_language_modeling}

Historically, language modeling has been a statistical task with probabilities of word occurrences calculated using data from large corpora \cite{Charniak1996,Jurafsky2008,Manning1999}. Initially, the bag-of-words approach was used, in which words were simply predicted by their frequencies of occurrence in the training corpus, possibly with smoothing of counts. A later development, that of the $n$-gram model, attempted to solve the problem by determining frequencies of words following each other. Inevitably, this significantly increased the size of the model and computation required to construct it, as instead of simply having vectors of size $v$, where $v$ was the size of the vocabulary, the models consisted of matrices of size $v \times v$. However, as many words rarely, if ever, follow each other in natural usage, the matrices were sparse. This observation allowed for significant reduction in the sizes of the models.

The $n$-gram approach does not simply look at the probabilities of words following single other words, but instead at the probabilities of words following a set of $n-1$ prior words. Hence, a bag-of-words model would be considered a unigram or 1-gram model, a model using only one previous word a 2-gram or bigram model, and a model using the two previous words a trigram model. Due to the decreasing likelihood of a set of words having co-occurred in the training corpus as the size of $n$ increases, a number of techniques were developed to allow for reasonably long $n$-grams to be used. \cite{Jurafsky2008} Typical models have used unigrams through 5-grams.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

SAMPLES = \
	sample-manuscript.tex \
	sample-acmsmall.tex \
	sample-acmlarge.tex \
	sample-acmtog.tex \
	sample-sigconf.tex \
	sample-sigconf-authordraft.tex \
	sample-sigplan.tex \
	sample-sigchi.tex \
	sample-sigchi-a.tex 


PDF = $(PACKAGE).pdf ${SAMPLES:%.tex=%.pdf} acmguide.pdf

all:  ${PDF}


%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do 	pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx  
	pdflatex $<

%.pdf:  %.tex   $(PACKAGE).cls ACM-Reference-Format.bst
	pdflatex $<
	- bibtex $*
	pdflatex $<
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done

sample-manuscript.pdf \
sample-acmsmall.pdf \
sample-acmlarge.pdf \
sample-acmtog.pdf: samplebody-journals.tex

sample-sigconf.pdf \
sample-sigconf-authordraft.pdf \
sample-sigplan.pdf \
sample-sigchi.pdf: samplebody-conf.tex


.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls


clean:
	$(RM)  $(PACKAGE).cls *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi

distclean: clean
	$(RM) $(PDF) *-converted-to.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

documents.zip: all
	zip $@ acmart.pdf acmguide.pdf sample-*.pdf


==> Overview/NeuralNetworks/Figures/CNNs.tex <==
\begin{figure*}%[t!]

    \centering
    
    \subfloat(a)
    %\begin{subfigure}
        %\centering
        \includegraphics[height=1.625in]{TablesAndFigures/CNN.png}
        %\caption{Basic CNN}
        \label{figure:simple_CNN}
    %\end{subfigure}
    \hfil
    \subfloat(b)
    %\begin{subfigure}
        %\centering
        \includegraphics[height=1.625in]{TablesAndFigures/CNN_with_pooling.png}
        %\caption{CNN with Pooling}
        \label{figure:CNN_with_pooling}
    %\end{subfigure}
    
    \caption{Convolutional Neural Networks. These networks have three distinct filters that operate on the input layer, each with a receptive field size of three. In (b), $k$-max pooling is exhibited, where $k = 2$ with a pool size of three.}
    
    \label{figure:CNNs}
    
\end{figure*}

%\begin{figure}[!t]
%\centering
%\includegraphics[width=2.5in]{myfigure}
%\caption{Simulation results for the network.}
%\label{fig_sim}
%\end{figure}

==> Overview/NeuralNetworks/Figures/LSTMs.tex <==
\begin{figure}[h!]

    \centering
    
    \includegraphics[width=2.5in]{TablesAndFigures/LSTM.png}
    
    \caption{Long Short-Term Memory Network. In this network, the input is concatenated with the previous output and is then distributed to an activation node and to three sigmoid  nodes followed by gate nodes. Depending on the outputs of the sigmoid nodes, the gate nodes choose whether or not to allow information to pass through. These gates control i) the input, ii) the recurrent internal state, and iii) the output.}
    
    \label{figure:LSTM}

\end{figure}

==> Overview/NeuralNetworks/Figures/RNNs.tex <==
\begin{figure*}[t!]

    \centering
    
    \subfloat(a)
    %\begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[width=1.75in]{TablesAndFigures/RNN.png}
        %\caption{Basic RNN}
        \label{figure:basic_RNN}
    %\end{subfigure}
    \hfil
    \subfloat(b)
    %\begin{subfigure}{0.67\textwidth}
        \centering
        \includegraphics[width=3.5in]{TablesAndFigures/stacked_RNN.png}
        %\caption{Stacked RNN}
        \label{figure:stacked_RNN}
    %\end{subfigure}
    \vfil
    \subfloat(c)
    %\begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[height=1in]{TablesAndFigures/RNN_unrolled.png}
        %\caption{Unrolled RNN}
        \label{figure:unrolled_RNN}
    %\end{subfigure}
    \hfil
    \subfloat(d)
    %\begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[height=1in]{TablesAndFigures/stacked_RNN_unrolled.png}
        %\caption{Unrolled RNN Stack}
        \label{figure:stacked_RNN_unrolled}
    %\end{subfigure}
    \hfil
    \subfloat(e)
    %\begin{subfigure}{0.33\textwidth}
        \centering
        \includegraphics[height=1in]{TablesAndFigures/bidirectional_RNN.png}
        %\caption{Bidirectional RNN}
        \label{figure:bidirectional_RNN}
    %\end{subfigure}
    
    \caption{Recurrent Neural Networks. These networks can be "unrolled" to appear as multiple different nodes. Note that (a) and (c) are identical, as are (b) and (d). If an entire data sequence is known prior to computation beginning, RNNs can also operate over the reverse sequence of the data. Bidirectional networks such as (e) utilize two RNNs working in opposite directions and then combine the outputs.}
    
    \label{figure:RNNs}

\end{figure*}

==> Overview/NeuralNetworks/Figures/SimpleNetworks.tex <==
\begin{figure*}%[t!]

    \centering
    
    \subfloat(a)
    %\begin{subfigure}{0.35\textwidth}
        %\centering
        \includegraphics[height=1.625in]{TablesAndFigures/dense_ANN.png}
        %\caption{Fully-Connected ANN}
        \label{figure:dense_ANN}
    %\end{subfigure}
    \hfil
    \subfloat(b)
    %\begin{subfigure}{0.25\textwidth}
        %\centering
        \includegraphics[height=1.625in]{TablesAndFigures/simple_ANN.png}
        %\caption{Non-dense ANN}
        \label{figure:basic_ANN}
    %\end{subfigure}
    \hfil
    \subfloat(c)
    %\begin{subfigure}{0.4\textwidth}
        %\centering
        \includegraphics[height=1.625in]{TablesAndFigures/ANN_with_hidden_layer.png}
        %\caption{ANN with Hidden Layer}
        \label{figure:ANN_with_hidden_layer}
    %\end{subfigure}
    
    
    \caption{Simple Neural Networks. Networks built until recently had very few layers. Early networks were fully connected as shown in (a), although non-dense networks, such as that shown in (b) are common these days. Layers that are neither the input nor output layers, as exhibited in (c), are said to be "hidden".}
    
    \label{figure:SimpleNetworks}
    
\end{figure*}
